Generative Models are Self-Watermarked: Declaring Model Authentication through Re-Generation

As machine- and AI-generated content proliferates, protecting the intellectual property of generative models has become imperative, yet verifying data ownership poses formidable challenges, particularly in cases of unauthorized reuse of generated data. The challenge of verifying data ownership is further amplified by using Machine Learning as a Service (MLaaS), which often functions as a black-box system. Our work is dedicated to detecting data reuse from even an individual sample. Traditionally, watermarking has been leveraged to detect AI-generated content. However, unlike watermarking techniques that embed additional information as triggers into models or generated content, potentially compromising output quality, our approach identifies latent fingerprints inherently present within the outputs through re-generation. We propose an explainable verification procedure that attributes data ownership through re-generation, and further amplifies these fingerprints in the generative models through iterative data re-generation. This methodology is theoretically grounded and demonstrates viability and robustness using recent advanced text and image generative models. Our methodology is significant as it goes beyond protecting the intellectual property of APIs and addresses important issues such as the spread of misinformation and academic misconduct. It provides a useful tool to ensure the integrity of sources and authorship, expanding its application in different scenarios where authenticity and ownership verification are essential.

==> conclusion.tex <==
\section{Conclusion}

In this work, we observe the intrinsic fingerprint in both text and vision generative models, which can be identified and verified by contrasting the re-generation of the suspicious data samples by authentic models and contrasting models. Furthermore, we propose iterative re-generation in the Generation Stage to enhance the fingerprints and provide a theoretical framework to ground the convergence of one-step re-generation distance by the authentic model. Our research paves the way towards a generalized authorship authentication for deep generative models without (1) modifying the original generative model, (2) post-processing to the generated outputs, or (3) an additional model for identity classification.

% \section{Discussion}
% paraphrasing




==> exp_cv.tex <==

\subsection{Image Generation Experiments} \label{subsec:ig_exp}
The main objective of the image generation task is to produce an image given a text prompt using a generative model. To generate the initial proposal of images, we sample 200 prompts each from the \textbf{MS-COCO dataset (COCO)}~\citep{lin2014microsoft} and \textbf{Polo Club Diffusion DB dataset (POLO)}~\citep{wang2022diffusiondb}, then we generate initial images corresponding to the prompts using all assigned models. We consider two settings in re-generating: {(1)} \textit{watermarking} images through inpainting and {(2)} \textit{fingerprinting} enhancement through full image re-generation. The subsequent paragraphs detail the methodologies for each.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures//One Step Discrimination/Density Distribution CLIP Polo.pdf}
    \caption{Density distribution of one-step re-generation among four image generation models on Polo Dataset. The authentic models from left to right are: 1) SD 2.1, 2) SDXL 1.0, 3) SD 2, 4) SDXL Base 0.9.}
    \label{fig:clip-one-step}
\end{figure*}



\paragraph{Watermarking through Inpainting}


% Image inpainting refers to filling in missing or masked regions of an image to reconstruct the original intact image. 
When re-generating authentic image $\vx$, we mask $1/N$-th ($N=10$) of its pixels with fixed positions as the watermark pattern. All pixels in the masked regions are then re-generated by inpainting using a generative model. 
Similar to text generation, the inpainting step is iterated multiple times, following Algorithm \ref{alg:gen_iter}. The comprehensive description of the watermarking procedure is provided in Appendix~\ref{app:watermark-detailed}. 
% We utilize the inpainting pipeline\footnote{\url{https://huggingface.co/docs/diffusers/api/pipelines/stable_diffusion/inpaint}} - StableDiffussion and StableDiffusionXL - provided by HuggingFace~\citep{von-platen-etal-2022-diffusers}}. 



\begin{figure*}
    \centering
    \includegraphics[width=1.\linewidth]{figures//CV Appendix//Image Regeneration Samples/SDXL09_Image_Regenerations - main_paper.pdf}
    \caption{The quality of fingerprinted images over multiple iterations of re-generation using SDXL 0.9B.}
    \label{fig:sdxl-0.9b-main}
\end{figure*}





% \vspace{-2mm}

\paragraph{Fingerprinting through Re-generation}  In the re-generation setting, we first split all possible mask positions into 8 non-overlapped sets, coined \textit{segments}, each with $1/8$ pixel positions for a given image $\vx_a$. We parallelly reconstruct each segment based on the rest $7/8$ pixels of the image as context. Then, we reassemble the 8 generated segments into a new full image $\vy$. When analyzing reconstructions of $\vy_a=\mathcal{G}_a(\vx_a) $ by contrasting models $\vy_c=\mathcal{G}_c(\vx_a)$, there is an expectation that models may exhibit variations in painting masked regions due to their inherent biases and training. In the verification stage, by comparing $\vy_a$ and $\vy_c$ to the original $\vx_a$, we aim to identify subtle model fingerprints based on the `edit-distance' from the original data to re-generated content.
For this study, each model generates 200 images, which are then re-generated over one to five iterations. We compute LPIPS and CLIP similarity between $\vx_a$ and $\vy$ to quantify the model behavior.\footnote{The performance of MSE and SSIM is reported in Appendix~\ref{app:convergence-regeneration}} The detailed discussion on the quality of re-generated images is provided in Appendix~\ref{app:image_regen_quality}. 



\textbf{Distance Convergence.} 
Similar to text re-generation, the re-generation distance converges for both watermarking and fingerprinting settings, as illustrated in Figures~\ref{fig:watermark-coco} and~\ref{fig:convergence-analysis-regen}, indicated by consistent downward trends across datasets and distance metrics. This implies that the re-generation process converges, with subsequent iterations yielding images that more closely resemble their predecessors. While our methodology proves efficacious in both scenarios, subsequent sections will prioritize the fingerprinting setting. Details about the watermarking setting can be found in Appendix \ref{app:convergence-watermark}.



% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/One Step Discrimination/Enhanced Regeneration Authentic Model Model 2 Coco Dataset CLIP.pdf}
%     \caption{Verifying data generated by authentic $\mathcal G_a$ SDv2.1 on Coco Dataset at various iterations.}
%     \label{fig:enhanced_disc_m2}
% \end{figure*}
\input{tables/tab_cv_verification_main}



\textbf{Discrepancy.}
In our study, we focus on the setting of iterative re-generation through inpainting and observe convergence that can reveal differences between models. Like the NLG section both authentic and contrast models perform a one-step re-generation of $\vx_a$ to obtain $\vy$ and the CLIP distance is measured between the outputs. 
As illustrated in \Figref{fig:clip-one-step}, the one-step re-generation density distribution of the authentic model predominantly peaks at lower values across $\mathcal{G}$. This indicates that authentic models can effectively distinguish their own re-generated outputs from those of non-authentic models. The divergence in CLIP distances after multiple rounds of inpainting highlights our method's ability to distinguish between generative models. Using images from later inpainting iterations (\eg $k>1$) further emphasizes each model's unique characteristics. A similar trend is evident with the Coco dataset and LPIPS distance metric, the details of which can be found in Appendix \ref{app:density_cv}.

The effectiveness of this method is illustrated in \Figref{fig:enhanced_disc_m2} where we can observe even generative models that are not adept at inpainting like SDv2.1 Base over iterations can successfully enhance their fingerprints by 5 iterations. While most models, on average, may require fewer rounds of re-generation to deeply impart their fingerprints, with more rounds of re-generation, even older models can successfully enhance their fingerprints. The quality of the images is illustrated in Fig~\ref{fig:sdxl-0.9b-main}, showcasing a high retention of visual quality through five iterations of re-generation, with the subject's features and the surrounding details remaining sharp and consistent. Simultaneously, the strength of the fingerprint of the generating model is reinforced over iterations, enhancing the model's traceability without degrading the image integrity, as indicated by the trend in Fig~\ref{fig:enhanced_disc_m2}. 




\textbf{Verification.} In accordance with the text generation framework, we utilize \Algref{alg:verify_process} to evaluate verification performance, selecting optimal parameters $k=5$ and $\delta=0.05$ based on the results of the text generation experiment. As demonstrated in \Tabref{tab:m2m_verification_clip}, models reliably identify images from the authentic model, with precision often exceeding 85\% and recall around 85\%.





==> exp_nlp.tex <==




\begin{figure*}[!htb]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/nlp/bleu_all_k1.pdf}
     \end{subfigure}
     \hfill
     \vspace{0.02cm}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/nlp/bleu_all_k5.pdf}
     \end{subfigure}
        \caption{Density distribution of one-step re-generation among four text generation models, where the input to the one-step re-generation is the $k$-th iteration from the authentic models. The authentic models from left to right are: 1) M2M, 2) mBART, 3) GPT3.5-turbo, and 4) Cohere.}
        \label{fig:bleu_one_step}
\end{figure*}


\subsection{Natural Language Generation Experiments} \label{subsec:nlg_exp}
% \xqk{The motivation is confusing here and raises me a question 'Can we use other paraphrase approach instead of RT?' (similar to one reviewer.)}
In the study of text generation, the primary objective is to produce sentences that fulfill specific requirements, including translation, paraphrasing, summarization, \etc. Then, one can re-generate intended output sentences via `paraphrasing' them. This study focuses on machine translation (specifically from French to English) as its primary generation task.\footnote{In addition to machine translation, we examine paraphrasing and summarization as the generation tasks in \Secref{sec:robustness}} Considering that \mone and \mtwo are restricted to machine translation tasks, we utilize round-trip translation to paraphrase English sentences. Specifically, for each round-trip translation step, an English input sentence is first translated into French and then back to English. %One can repeat this process as depicted in~\Algref{alg:gen_iter} until the resultant sentence stabilizes. 
We repeat this process multiple times to observe the change of the `edit' distances.
For \mthree and \mfour, we perform all experiments in a zero-shot prompting. We use the following prompts:
\begin{itemize}
    \item Translate to English: \textit{You are a professional translator. You should translate the following sentence to English and output the final result only: \{\textbf{INPUT}\}}
    \item Translate to French: \textit{You are a professional translator. You should translate the following sentence to French and output the final result only: \{\textbf{INPUT}\}}
\end{itemize}


\input{tables/tab_nlp_verification_diff_rate}
\input{tables/tab_nlp_verification}

It has been known that text generative models exhibit superior performance when test data inadvertently overlaps with pre-training data, a phenomenon referred to as data contamination~\citep{magar2022data}. To address this potential issue, we sample 200 sentences from the in-house data as the starting point for each model. To mitigate biases stemming from varied sampling strategies, we set the temperature and top p to 0.7 and 0.95 for all models and experiments. 
% Comprehensive settings for this generation process are provided in Appendix~\ref{app:text_gen_setting}.





% \xqk{Move Fig 2 to this page.}
\paragraph{Distance Convergence.} The dynamics of the distance change across three metrics and various generative models are depicted in \Figref{fig:self_iter_nlp}. We observe a remarkable distance reduction between the first and second iterations in all settings. Subsequently, the changes in distance between consecutive iterations exhibit a diminishing pattern, tending to converge after approximately 5-7 rounds of re-generation. These observed trends are consistent with the fixed-point theorem as elaborated in \Secref{sec:fixed_point}.




\paragraph{Discrepancy.} In our study of iterative re-generation using the same model, we observe convergence which can be utilized to distinguish the authentic model from its counterparts. As delineated in \Secref{subsec:regeneration}, for each sentence $\vx$ from our corpus $X$, we apply the authentic model to yield $\vx_a$ via a translation. Both authentic and contrasting models then perform a one-step re-generation of $\vx_a$ to obtain $y$. Finally, we can measure the distance between $\vx_a$ and $\vy$ (including $\vy_a$ and $\vy_c$) as described in \Secref{subsec:regeneration}. According to \Figref{fig:bleu_one_step}, the density distribution associated with the authentic model demonstrates a noticeable divergence from those of models for contrast, thus affirming the hypothesis discussed in \Secref{subsec:regeneration}. This consistent pattern holds when using ROUGE-L and BERTScore for distance measures, as evidenced by their respective density distributions in Appendix~\ref{app:density}. 


\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures//Distance Convergence Regeneration/Convergence Regnerated Images.pdf}
    \caption{The convergence analysis of the distances in iterations based on CLIPS and LPIPS metrics on re-generated images of 200 samples on Coco and Polo datasets.}
    \label{fig:convergence-analysis-regen}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/One Step Discrimination/Enhanced Regeneration Authentic Model Model 2 Coco Dataset CLIP.pdf}
    \includegraphics[width=0.9\linewidth]{figures/One Step Discrimination/Enhanced Regeneration Authentic Model Model 7 Coco Dataset CLIP.pdf}
    \caption{Verifying data generated by authentic $\mathcal G_a$ SDv2.1 and SDv 2.1 Base on Coco Dataset at various iterations using CLIP distance.}
    \label{fig:enhanced_disc_m2}
    \vspace{-3mm}
\end{figure*}


% \xqk{Cohere does not look good. Shall we use some better examples or explain this phenomena?} \xuanli{this is because of poor translation performance compared to other models. I mentioned this phenomenon in footnote 6}
We observe the difficulty of distinguishing Cohere from other models merely based on the outputs from the first iteration, \ie without re-generation. We attribute the distinctive behavior of Cohere to its relatively slower convergence than other models.\footnote{The underlying reason behind the slow convergence for Cohere is investigated in Appendix~\ref{app:text_regen}.} However, as depicted in \Figref{fig:self_iter_nlp}, the distances observed in subsequent iterations of the same model experience a substantial reduction. This implies the re-generated outputs in the Generation Stage possess enhanced fingerprints. In particular, we can derive $x_a^{\langle k \rangle}$ from $5$ iterations of $\mathcal{G}_a(\cdot)$. \Figref{fig:bleu_one_step} shows that increasing $k$ enhances the differentiation of the authentic model's density distribution compared to other models. This distinction becomes evident even in the case of Cohere, which remains indistinguishable at $k=1$. This enhancement for Cohere is also corroborated in the verification part.



\paragraph{Verification.} We employ \Algref{alg:verify_process} to ascertain if a given sentence originates from the authentic models. The determination hinges on the threshold parameter, $\delta$. Thus, we designate \mone as the authentic model, while using \mtwo, \mfour, and \mthree as contrast models to determine the optimal value of $\delta$. As indicated in \Tabref{tab:m2m_verification}, a threshold of 0.05 certifies that the three contrast models can validate that more than 93\% of the samples are derived from \mone. As anticipated, an increase in the value of $\delta$ augments the stringency criteria, resulting in a reduction in verification precision. Therefore, we fix $\delta$ at 0.05 for ensuing evaluations unless stated otherwise.





As indicated in \Tabref{tab:ACC_all_nlp_models}, our approach undertakes the validation of authorship, yielding a precision exceeding 85\% and a recall rate surpassing 88\% across \mone, \mtwo, and \mthree. Moreover, both precision and recall metrics improve with additional re-generation iterations. 
As expected, Cohere's slower convergence results in comparatively less effective performance. Nevertheless, enhancements in both precision and recall are observed when $k=5$.




==> exp_robustness.tex <==
\input{tables/tab_paraphrasing}


\subsection{Generalization and Robustness Evaluation}
\label{sec:robustness}
\paragraph{Task Generalization} To demonstrate the generalization of our approach, we further examine two popular text generation tasks using prompting: paraphrasing and summarization. The corresponding prompts are:
\begin{itemize}
    \item \textbf{paraphrasing}: \textit{You are a professional language facilitator. You should paraphrase the following sentence and output the final result only:};
    \item \textbf{Summarization}: \textit{You are a professional language facilitator. You should summarize the following document using one sentence:}
\end{itemize}
We use prompt-based paraphrasing for one-step re-generation, opting for a $k$ value of 5 due to its superior performance. As for backbone models for text generation tasks, we consider \mthree, Llama2-chat-7B~\cite{touvron2023llama}, and Mistral~\cite{jiang2023mistral}.

\Tabref{tab:add_nlp_tasks} demonstrates that while paraphrasing and summarization tasks exhibit performance degradation compared to machine translation, our approach effectively distinguishes IPs among various models. This supports the overall effectiveness of our approach across a wide range of text-generation tasks.





Until now, we assumed that malicious users employed the authentic model to generate text and images, subsequently utilizing and disseminating them directly. Nevertheless, in order to circumvent potential IP infringements, malicious users may choose to modify the generated content prior to its public dissemination. This situation poses a challenge to the effectiveness of our approach in protecting the IP claims associated with the altered content.

\paragraph{Robustness Evaluation} To assess the robustness of our verification process, we simulate the modification process using paraphrasing and perturbation attacks.

Our robustness assessment commenced with a paraphrasing attack targeting image generation. This experiment was designed to test the efficacy of our verification process in identifying plagiarized images. Specifically, we use a set of images designated as $A\_B$, originally generated by one model (Model A) and then re-generated or paraphrased by another model (Model B). We experiment with SD v2.1 as the authentic model and SDXL 1.0 as the paraphrasing model. 
 

We re-generate these paraphrased $A\_B$ images using both the authentic and paraphrasing models to analyze the distance density distribution variations. Furthermore, we assess this paraphrasing attack at different rounds of generation $\vx_a^{\langle K\rangle}$ where K is 1, 3, and 5 by the authentic model. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures//CV paraphrasing/Density Distribution paraphrase SDv2-1 with contrast.pdf}
    \caption{The variations in distance density distribution between paraphrased images and the authentic model, paraphrasing model and a contrast model which is not involved in the generation process of the paraphrased images. The paraphrased images are initially generated by SDv2.1 (authentic model) and then paraphrased by models SDXL 1.0 at different rounds of K (1, 3 \& 5) by the authentic model. Additionally, SDv2 acts as a contrast model for the set of images which is produced by SDv2.1 and then paraphrased by SDXL 1.0. }
    \label{fig:density-distribution-comparison-paraphrase}
    \vspace{-4mm}
\end{figure}

The results, represented in ~\Figref{fig:density-distribution-comparison-paraphrase}, show comparisons such as $\mathbb{D}(A\_B, \mathcal{G}_A(A\_B))$ and $\mathbb{D}(A\_B, \mathcal{G}_B(A\_B))$, indicating the distance between the paraphrased image (created by A then paraphrased by B) and re-generated images.

% The analysis reveals that the peak density with the authentic model is higher and at a lower distance compared to the adversarial model, suggesting subtle differences in the paraphrasing abilities of the models. 
We observe a significant challenge in attributing authorship to the original creator model once the image is plagiarized (even at higher values of re-generation iteration K in Algorithm~\ref{alg:gen_iter}). The distance between the paraphrased image to the authentic model and the paraphrasing model cannot be differentiated making it increasingly difficult to distinguish whether the SDv2.1 model or another paraphrasing model generated the image. 
This overlap in the density distributions is a limitation in our methodology, which relies on discerning the nuances in these distances for authorship attribution. This is a common weakness of any fingerprinting or watermarking methods where there is no provable robustness guarantee ~\cite{10.1145/3576915.3623189}. 

% \xqk{Shall we cite papers here?}

However, the results also reveal a noteworthy strength in the methodology. There is a discernible and consistently large distance when comparing paraphrased images to those generated by a contrast model (\ie an unrelated model, one which was neither the authentic nor the paraphrasing model). This finding is crucial as it suggests that despite the challenges in direct attribution, our approach can reliably detect when an external model, not involved in the image's original creation or its paraphrasing, is falsely claimed as the author. Therefore, this method could potentially be leveraged to establish joint authorship in scenarios where the paraphrased image is claimed by a third party, ensuring proper credit is given to the authentic and paraphrasing models involved in the image's creation.  


We investigate perturbation attacks in both text and image generation tasks. For our NLP experiments, we randomly perturb $X$\% of the words preceding the one-step re-generation procedure by substituting them with random words. The value of $X$ ranges from 10\% to 50\%. We designate \mthree as the authentic model. We set $k=5$, due to its outperforming performance. As depicted in \Tabref{tab:nlp_robustness_evaluation}, as the perturbation rate increases, we observe a gradual decline in the verification performance of our method. In general, the efficacy of watermark verification remains reasonably positive. Nevertheless, we argue that perturbations in the range of 30\% to 50\% have a notable adverse impact on the quality of the generated texts, rendering them significantly less valuable for potential attackers.

\input{tables/tab_nlp_robustness}



Regarding image generation, we introduce two types of perturbations: Gaussian Noise and Brightness alterations.
In the first robustness experiment, Gaussian noise is applied to a random subset of pixels (r) in the original image before re-generation, using a fixed mean ($\mu$ = 0) and standard deviation ($\sigma$ = 4). The second robustness assessment involves modifying the brightness of 10\% of randomly selected pixels in the images. As expected, as the perturbation intensity increases, our verification precision decreases. When we introduced Gaussian noise to different proportions of pixels, we observed minimal impact on verification accuracy across various models, as evidenced in \Tabref{tab:robustness_evaluation}. Even at a 50\% noise level, the models maintained a precision range of 89-99\%. This highlights the robustness of the proposed approach, even in the presence of high levels of random noise. In contrast, brightness perturbations reveal that the watermark is more sensitive to changes in brightness than to Gaussian noise. Examining \Tabref{tab:brightness_evaluation}, we observe a sharp decline in precision for SDXL 1.0, which remains relatively stable until a perturbation rate of 1.02. Beyond this threshold, the model's robustness is significantly compromised.

\input{tables/tab_cv_robustness_noise}
\input{tables/tab_cv_robustness_brightness}

\paragraph{Distance Differentiation between Natural and AI-Generated Images} In order to assess the viability of our framework to detect plagiarism on naturally made images (i.e., shot on camera), we re-generate natural images from the MS COCO 2017 Evaluation set \cite{lin2014microsoft} with previously used image generation models for one iteration. We compare the Clip distances between these natural images and their respective re-generations to the distance between the AI-generated images and their re-generation for one iteration by the corresponding models as presented in ~\Figref{fig:Comparison of Density Distribution of Distances Natual vs AI Image Regenerations}. There is a clear distinction in the distance density distribution when AI-generated images are re-generated using AI our Generation Algorithm \ref{alg:gen_iter}, the distance remains low whereas using a natural image for re-generation results in further distances even with the most advanced AI models.




\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Density Distribution Natural vs AI Images.pdf}
    \caption{Comparison of Density Distribution of Re-generation Distances in Verification Stage, acquired by Natural vs AI Image Re-generations.} 
    
    % \xqk{Over to exp section and it should be before Fig 8.}}
    \label{fig:Comparison of Density Distribution of Distances Natual vs AI Image Regenerations}
\end{figure}



==> sec5_discussion.tex <==
\section{Discussion}
% paraphrasing

The experiments demonstrate that iterative image regeneration can be an effective method for detecting image generation model fingerprints and enabling source verification. Specifically, regenerating images multiple times allows subtle biases and differences between models to become more pronounced and detectable. We observe consistent convergence and decreasing distance metrics across datasets and models, indicating the regeneration process enhances model-specific fingerprints. 


While we have observed the method being susceptible to paraphrasing attacks, a notable strength is that there is scope to jointly attribute ownership to both models involved in the creation process while successfully being able to differentiate between a model that was not involved in the generation process. 
The robustness evaluations indicated the verification is resilient to perturbations like noise and brightness changes. Comparisons to natural images demonstrated the potential to differentiate AI-generated images from natural images thereby showing promise to detect deepfakes.
Overall, iterative regeneration enables subtle model biases to compound into detectable fingerprints. As models continue to advance in quality and realism, regeneration-based fingerprinting provides a promising direction for authentication and protecting against misuse. Further research can refine these techniques and examine their effectiveness across diverse datasets and state-of-the-art models.

==> tables/tab_thresh_SD2.1.tex <==
\begin{table}[h]
    \centering
    \inserttxt{\caption{The accuracy of differentiating contrast models from the authentic model SDv2.1 using different $\delta$.}}
    \scalebox{0.98}{
    \begin{tabular}{c|cccc}
    \toprule
    \multirow{2}{*}{\textbf{$\delta$}} & \multicolumn{4}{c}{\textbf{SDv2.1}} \\
    & \textbf{SD v2.} & \textbf{SD v2.1B} & \textbf{SDXL 0.9} & \textbf{SDXL 1.0} \\
    \midrule
    0.05 & 0.990 & 1.00 & 1.00 & 1.00 \\
    0.10 & 0.985 & 1.00 & 1.00 & 1.00 \\
    0.20 & 0.960 & 1.00 & 1.00 & 1.00 \\
    0.40 & 0.895 & 1.00 & 0.995 & 0.985 \\

    \bottomrule
    \end{tabular}
    }
    \label{tab:cv_verification_SDv2.1}
\end{table}
